Data Provision to an Informed Seller

A monopoly seller is privately and imperfectly informed about the buyer's value of the product. The seller uses information to price discriminate the buyer. A designer offers a mechanism that provides the seller with additional information based on the seller's report about her type. We establish the impossibility of screening for welfare purposes, i.e., the designer can attain any implementable combination of buyer surplus and seller profit by providing the same signal to all seller types. We use this result to characterize the set of implementable welfare outcomes, study the seller's incentive to acquire third-party data, and demonstrate the trade-off between buyer surplus and efficiency.

==> macros.tex <==
\newcommand{\type}{\ensuremath{\theta}}
\newcommand{\typeb}{\ensuremath{t}}
\newcommand{\typedist}{\ensuremath{f}}
\newcommand{\typemeas}{\ensuremath{F}}
\newcommand{\density}{\ensuremath{f}}
\newcommand{\types}{\ensuremath{\Theta}}
\newcommand{\typesb}{\ensuremath{T}}
\newcommand{\wtp}{\ensuremath{v}}
\newcommand{\wtps}{\ensuremath{V}}
%\newcommand{\value}{\ensuremath{v}}
%\newcommand{\values}{\ensuremath{V}}
%\newcommand{\signal}{\ensuremath{\info}}
\newcommand{\price}{\ensuremath{p}}
\newcommand{\map}{\ensuremath{\mathcal{\pi}}}
\newcommand{\tran}{\ensuremath{t}}
\newcommand{\monopolyprofit}{\ensuremath{\Pi}}
\newcommand{\consumersurplus}{\ensuremath{U}}
\newcommand{\cs}{\ensuremath{\text{\textup{U}}}}
\newcommand{\profit}{\ensuremath{\Pi}}
\newcommand{\reals}{\ensuremath{\mathbb{R}}}
\newcommand{\info}{\ensuremath{\mathcal{I}}}
\newcommand{\noinfo}{\ensuremath{\underline{\mathcal{I}}}}
\newcommand{\fullinfo}{\ensuremath{\overline{\mathcal{I}}}}
\newcommand{\implementable}{\ensuremath{\mathcal{S}}}
\newcommand{\rec}{\ensuremath{r}} %recommendation
\newcommand{\high}{\ensuremath{H}} %high WTP
\newcommand{\low}{\ensuremath{L}} %low WTP
\newcommand{\med}{\ensuremath{M}} %medium WTP
\newcommand{\typetr}{\ensuremath{\hat{\theta}}}
\newcommand{\typetrpost}{\ensuremath{\tilde{\theta}}}
\newcommand{\belief}{\ensuremath{\mu}}
\newcommand{\prior}{\ensuremath{\belief_0}}
\newcommand{\signal}{\ensuremath{s}}
\newcommand{\signals}{\ensuremath{S}}
\newcommand{\post}{\ensuremath{t}}
\newcommand{\dint}{\ensuremath{\mathrm{d}}}
\newcommand{\eqmset}{\ensuremath{\mathcal{E}}}
\newcommand{\csmin}{\ensuremath{\underline{\cs}}}
\newcommand{\menu}{\ensuremath{\mathcal{M}}}

% \newcommand{\ubar}[1]{\underaccent{\bar}{#1}}
% \newcommand{\field}[1]{\mathbb{#1}}
% \newcommand{\set}[1]{\mathcal{#1}}
 \newcommand{\R}{\ensuremath{\mathbb{R}}}
 \newcommand{\E}{\ensuremath{\mathbb{E}}}
% \newcommand{\PP}{\mathbf{P}}
% \newcommand{\DD}{\mathcal{D}}
% \newcommand{\argmax}[1]{\underset{#1}{\operatorname{arg}\,\operatorname{max}}\;}

\newcommand{\prot}{\ensuremath{\mathcal{P}}}
\newcommand{\stratb}{\ensuremath{\sigma_B}}
\newcommand{\strats}{\ensuremath{\sigma_S}}
\newcommand{\stratsb}{\ensuremath{\Sigma_B}}
\newcommand{\stratss}{\ensuremath{\Sigma_S}}
\newcommand{\ab}{\ensuremath{a_B}}
\newcommand{\as}{\ensuremath{a_S}}
\newcommand{\asb}{\ensuremath{A_B}}
\newcommand{\ass}{\ensuremath{A_S}}
